The Arctic Circle Revisited

The problem of limit shapes in the six-vertex model with domain wall boundary conditions is addressed by considering a specially tailored bulk correlation function, the emptiness formation probability. A closed expression of this correlation function is given, both in terms of certain determinant and multiple integral, which allows for a systematic treatment of the limit shapes of the model for full range of values of vertex weights. Specifically, we show that for vertex weights corresponding to the free-fermion line on the phase diagram, the emptiness formation probability is related to a one-matrix model with a triple logarithmic singularity, or Triple Penner model. The saddle-point analysis of this model leads to the Arctic Circle Theorem, and its generalization to the Arctic Ellipses, known previously from domino tilings.

==> fig-dwbcgrid.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% figure 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\unitlength=1mm
\begin{center}
\begin{picture}(30,30)
\put(0,5){\line(1,0){30}}
\put(5,5){\vector(-1,0){3.5}}
\put(10,5){\vector(-1,0){3.5}}
\put(15,5){\vector(-1,0){3.5}}
\put(20,5){\vector(-1,0){3.5}}
\put(25,5){\vector(-1,0){3.5}}
\put(25,5){\vector(1,0){3.5}}
%
\put(0,10){\line(1,0){30}}
\put(5,10){\vector(-1,0){3.5}}
\put(10,10){\vector(-1,0){3.5}}
\put(10,10){\vector(1,0){3.5}}
\put(15,10){\vector(1,0){3.5}}
\put(20,10){\vector(1,0){3.5}}
\put(25,10){\vector(1,0){3.5}}
%
\put(0,15){\line(1,0){30}}
\put(5,15){\vector(-1,0){3.5}}
\put(10,15){\vector(-1,0){3.5}}
\put(15,15){\vector(-1,0){3.5}}
\put(20,15){\vector(-1,0){3.5}}
\put(20,15){\vector(1,0){3.5}}
\put(25,15){\vector(1,0){3.5}}
%
\put(0,20){\line(1,0){30}}
\put(5,20){\vector(-1,0){3.5}}
\put(5,20){\vector(1,0){3.5}}
\put(15,20){\vector(-1,0){3.5}}
\put(15,20){\vector(1,0){3.5}}
\put(20,20){\vector(1,0){3.5}}
\put(25,20){\vector(1,0){3.5}}
%
\put(0,25){\line(1,0){30}}
\put(5,25){\vector(-1,0){3.5}}
\put(10,25){\vector(-1,0){3.5}}
\put(10,25){\vector(1,0){3.5}}
\put(15,25){\vector(1,0){3.5}}
\put(20,25){\vector(1,0){3.5}}
\put(25,25){\vector(1,0){3.5}}
%
\put(5,0){\line(0,1){30}}
\put(5.05,0){\vector(0,1){3.5}}
\put(5.05,5){\vector(0,1){3.5}}
\put(5.05,10){\vector(0,1){3.5}}
\put(5.05,15){\vector(0,1){3.5}}
\put(5.05,25){\vector(0,-1){3.5}}
\put(5.05,30){\vector(0,-1){3.5}}
%
\put(10,0){\line(0,1){30}}
\put(10.05,0){\vector(0,1){3.5}}
\put(10.05,5){\vector(0,1){3.5}}
\put(10.05,15){\vector(0,-1){3.5}}
\put(10.05,20){\vector(0,-1){3.5}}
\put(10.05,20){\vector(0,1){3.5}}
\put(10.05,30){\vector(0,-1){3.5}}
%
\put(15,0){\line(0,1){30}}
\put(15.05,0){\vector(0,1){3.5}}
\put(15.05,5){\vector(0,1){3.5}}
\put(15.05,10){\vector(0,1){3.5}}
\put(15.05,15){\vector(0,1){3.5}}
\put(15.05,25){\vector(0,-1){3.5}}
\put(15.05,30){\vector(0,-1){3.5}}
%
\put(20,0){\line(0,1){30}}
\put(20.05,0){\vector(0,1){3.5}}
\put(20.05,5){\vector(0,1){3.5}}
\put(20.05,10){\vector(0,1){3.5}}
\put(20.05,20){\vector(0,-1){3.5}}
\put(20.05,25){\vector(0,-1){3.5}}
\put(20.05,30){\vector(0,-1){3.5}}
%
\put(25,0){\line(0,1){30}}
\put(25.05,0){\vector(0,1){3.5}}
\put(25.05,10){\vector(0,-1){3.5}}
\put(25.05,15){\vector(0,-1){3.5}}
\put(25.05,20){\vector(0,-1){3.5}}
\put(25.05,25){\vector(0,-1){3.5}}
\put(25.05,30){\vector(0,-1){3.5}}
%
\put(12.5,-4){(a)}
\end{picture}
\qquad\qquad
\begin{picture}(30,30)
\put(0,5){\line(1,0){30}}
\put(0,10){\line(1,0){30}}
\put(0,15){\line(1,0){30}}
\put(0,20){\line(1,0){30}}
\put(0,25){\line(1,0){30}}
%
\put(5,0){\line(0,1){30}}
\put(10,0){\line(0,1){30}}
\put(15,0){\line(0,1){30}}
\put(20,0){\line(0,1){30}}
\put(25,0){\line(0,1){30}}
\linethickness{0.5mm}
%
\put(0,5){\line(1,0){25.25}}
\put(25,30){\line(0,-1){25.25}}
%
\put(0,10){\line(1,0){10.25}}
\put(20,30){\line(0,-1){15.25}}
\put(20.25,14.75){\line(-1,0){10}}
\put(10.25,9.75){\line(0,1){5.25}}
%
\put(0,15.25){\line(1,0){10}}
\put(15,30){\line(0,-1){10.25}}
\put(15,20){\line(-1,0){5.5}}
\put(9.75,20){\line(0,-1){5}}
%
\put(0,20){\line(1,0){5.25}}
\put(10,30){\line(0,-1){5.25}}
\put(10.25,24.75){\line(-1,0){5}}
\put(5.25,25){\line(0,-1){5.25}}
%
\put(0,25.25){\line(1,0){5}}
\put(4.75,30){\line(0,-1){5}}
%
%
\put(12.5,-4){(b)}
\end{picture}
\end{center}




==> fig-ffpcorr.tex <==
\psset{unit=.75cm,dotsep=.1,arrowscale=2,dotscale=1.5}
\begin{pspicture}(0,0)(9,10.5)
%\psframe(0,-1)(9,10)
\multips(1,0)(1,0){8}{\psline(0,0)(0,3.2)}
\multips(0,1)(0,1){8}{\psline(0,0)(2.2,0)}
\multips(3,1)(0,1){8}{\psline(-.2,0)(3.2,0)}
\multips(1,9)(1,0){8}{\psline(0,0)(0,-5.2)}
\multips(9,1)(0,1){8}{\psline(0,0)(-2.2,0)}
%
\multips(1,3.3)(1,0){8}{\psline[linestyle=dotted](0,0)(0,.4)}
\multips(2.3,1)(0,1){8}{\psline[linestyle=dotted](0,0)(.4,0)}
\multips(6.3,1)(0,1){8}{\psline[linestyle=dotted](0,0)(.4,0)}
%
\multirput(1,.25)(1,0){8}{\psline{->}(0,0)(0,.5)}
\multirput(.25,1)(0,1){8}{\psline{<-}(0,0)(.5,0)}
\multirput(1,8.75)(1,0){8}{\psline{->}(0,0)(0,-.5)}
\multirput(8.75,1)(0,1){8}{\psline{<-}(0,0)(-.5,0)}
\rput(4.25,8){\psline{<-}(0,0)(.5,0)}
\rput(4.25,7){\psline{<-}(0,0)(.5,0)}
\rput(4.25,6){\psline{<-}(0,0)(.5,0)}
\rput(4.25,5){\psline{<-}(0,0)(.5,0)}
%
\rput(5.1,9.5){$r$}
\rput(8,9.5){$1$}
\psline{->}(7.5,9.5)(5.5,9.5)
%
\rput(9.6,5){$s$}
\rput(9.6,8){$1$}
\psline{->}(9.6,7.5)(9.6,5.5)
\end{pspicture}




==> fig-vertices.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% Figure 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\unitlength=1mm
\begin{center}
\begin{picture}(124,30)
% ARROWS
% vertex a1
\put(7,20){\line(0,1){10}}
\put(7,22.5){\vector(0,-1){1}}
\put(7,27.5){\vector(0,-1){1}}
\put(2,25){\line(1,0){10}}
\put(4.5,25){\vector(-1,0){1}}
\put(9.5,25){\vector(-1,0){1}}
% vertex a2
\put(27,20){\line(0,1){10}}
\put(27,22.5){\vector(0,1){1}}
\put(27,27.5){\vector(0,1){1}}
\put(22,25){\line(1,0){10}}
\put(24.5,25){\vector(1,0){1}}
\put(29.5,25){\vector(1,0){1}}
% vertex b1
\put(52,20){\line(0,1){10}}
\put(52,22.5){\vector(0,-1){1}}
\put(52,27.5){\vector(0,-1){1}}
\put(47,25){\line(1,0){10}}
\put(49.5,25){\vector(1,0){1}}
\put(54.5,25){\vector(1,0){1}}
% vertex b2
\put(72,20){\line(0,1){10}}
\put(72,22.5){\vector(0,1){1}}
\put(72,27.5){\vector(0,1){1}}
\put(67,25){\line(1,0){10}}
\put(69.5,25){\vector(-1,0){1}}
\put(74.5,25){\vector(-1,0){1}}
% vertex c1
\put(97,20){\line(0,1){10}}
\put(97,22.5){\vector(0,1){1}}
\put(97,27.5){\vector(0,-1){1}}
\put(92,25){\line(1,0){10}}
\put(94.5,25){\vector(-1,0){1}}
\put(99.5,25){\vector(1,0){1}}
% vertex c2
\put(117,20){\line(0,1){10}}
\put(117,22.5){\vector(0,-1){1}}
\put(117,27.5){\vector(0,1){1}}
\put(112,25){\line(1,0){10}}
\put(114.5,25){\vector(1,0){1}}
\put(119.5,25){\vector(-1,0){1}}
% LINES
% vertex a1
\linethickness{0.5mm}
\put(7.25,10.25){\line(0,1){4.75}}
\put(7.5,10.25){\line(-1,0){5}}
\put(7.75,9.75){\line(0,-1){4.75}}
\put(7.5,9.75){\line(1,0){5}}
% vertex a2
\thinlines
\put(27,5){\line(0,1){10}}
\put(22,10){\line(1,0){10}}
% vertex b1
\linethickness{0.5mm}
\put(51.75,5){\line(0,1){10}}
\thinlines
\put(47,10){\line(1,0){10}}
% vertex b2
\thinlines
\put(72,5){\line(0,1){10}}
\linethickness{0.5mm}
\put(67,9.75){\line(1,0){10}}
% vertex c1
\linethickness{0.5mm}
\put(96.75,10){\line(0,1){5}}
\put(96.9,10){\line(-1,0){5}}
\thinlines
\put(97,9.75){\line(0,-1){5}}
\put(97,9.7){\line(1,0){4.7}}
% vertex c2
\put(117,10.25){\line(0,1){4.75}}
\put(117,10.25){\line(-1,0){5}}
\linethickness{0.5mm}
\put(117.25,10){\line(0,-1){4.75}}
\put(117,10){\line(1,0){5}}
% WEIGHTS
\put(5,-3){$w_1$}
\put(25,-3){$w_2$}
\put(50,-3){$w_3$}
\put(70,-3){$w_4$}
\put(95,-3){$w_5$}
\put(115,-3){$w_6$}
\end{picture}
\end{center}




